Simulations of the nEDM@SNS light collection system efficiency

A system for collecting the scintillation light produced by the capture process of ultra-cold neutrons (UCN) on polarized $^{3}$He is discussed and results from simulations of its performance are presented. This system will be implemented in nEDM@SNS, the experiment searching for the neutron electric dipole moment (nEDM) at the Spallation Neutron Source (SNS) at Oak Ridge National Laboratory. Simulation results show that the light collection system collects on average 17 photoelectrons per UCN-$^{3}$He capture event (sufficient to generate a robust signal), reconstructs the event location in the beam direction to approximately 3 cm accuracy, detects capture events with a high and spatially uniform efficiency (0.95 with 1% variation), and rejects greater than 50% of beta decay background events.

==> acknowledgements.tex <==
\section*{Acknowledgements} \label{sec:acknowledgements}
The authors would like to thank John Ramsey for the set of light collection system CAD models and Takeyasu Ito and Kent Leung for their support in the development of the light collection system simulation. The authors would also like  to thank Leah Broussard, Bob Golub, Steve Lamoreaux, and Mike Hayden for their discussion and suggestions. This work was supported in part by the U.S. Department of Energy, Office of Science, Office of Workforce Development for Teachers and Scientists (WDTS) under the Science Undergraduate Laboratory Internship program.
